Explainable Planning

As AI is increasingly being adopted into application solutions, the challenge of supporting interaction with humans is becoming more apparent. Partly this is to support integrated working styles, in which humans and intelligent systems cooperate in problem-solving, but also it is a necessary step in the process of building trust as humans migrate greater responsibility to such systems. The challenge is to find effective ways to communicate the foundations of AI-driven behaviour, when the algorithms that drive it are far from transparent to humans. In this paper we consider the opportunities that arise in AI planning, exploiting the model-based representations that form a familiar and common basis for communication with users, while acknowledging the gap between planning algorithms and human problem-solving.

==> applications.tex <==
\section{Practical Applications}

\dan{Mention multiple-battery managements}

\dan{Mention AUV scenario from San Diego}

\dan{Mention multi-drone base patrolling}

\dan{Mention smart-grid example from Derek}

==> graph.tex <==
\begin{center}
	\begin{tabular}{ l l l}
	
	   
	
	\begin{minipage}{0.12\textwidth}                   
	 \begin{tikzpicture}[->,auto,node distance=2.0cm, thick, scale=0.8]
	                    
	  \tikzstyle{every state}=[fill=orange,draw=none,text=white, scale=0.25]
	  \tikzstyle{blue edge} = [draw,line width=0.25pt,blue]
	  \tikzstyle{edge} = [draw,line width=0.25pt,green]
	
	
	  \node[state] (A)                    {};
	  \node[state]         (B) [above right of=A] {};
	  \node[state]         (D) [below right of=A] {};
	  \node[state]         (C) [below right of=B] {};
	  \node[state]         (E) [below of=D]       {};
	  \node[state]         (F) [right of=D]       {};
	  \node[state]         (G) [below of=B]       {};
	  \node[state]         (H) [below right of=D] {};
	  \node[state]         (I) [below right of=H] {};
	  \node[state]         (J) [above right of=I] {};
	  \node[state]         (K) [above right of=C] {};
	  \node[state]         (L) [right of=C] {};
	  \node[state]         (M) [below right of=J] {};
	  \node[state]         (N) [ right of=M] {};
	  \node[state]         (NJ)[above right of=N] {};
	  \node[state]         (O) [above  of=NJ] {};
	  \node[state]         (P) [above left of=O] {};
	  \node[state]         (Q) [below left of=P] {};
	  \node[state]         (R) [above of=P] {};
	  \node[state]         (X) [below of=Q] {};
	  \node[state]         (Y) [left of=R] {};
	  
	  %\draw (A)--(Q);
	
	  \path (A) [blue edge]  [bend left]    node {} (B)
	            edge [bend left]  node {} (C)
	            
	            edge [bend right]  node {} (L)
	        (B) edge [bend left]  node {} (C)
	            
	            edge [bend left]  node {} (I)
	            
	            edge [bend right]  node {} (F)
	        (C) edge [bend left]  node {} (D)
	            
	            edge [bend left]  node {} (P)
	            
	            edge [bend right]  node {} (NJ) 
	        (D) edge [bend left]  node {} (A)
	           
	            edge [bend right]  node {} (NJ)
	            
	         (E) edge [bend right]  node {} (P)
	            
	            edge [bend right]  node {} (G)
	           
	          (F) edge [bend right]  node {} (P)
	            edge [bend right]  node {} (I)
	          
	            edge [bend right]  node {} (NJ)
	          (G)
	            edge [bend left]  node {} (A)
	            edge [bend left]  node {} (B)
	            edge [bend left]  node {} (C)
	          
	            
	          (I) 
	            
	            
	            edge [bend left]  node {} (D)
	         
	            edge [bend right]  node {} (F)
	            
	            (K) edge [bend left]  node {} (A)
	            edge [bend left]  node {} (P)
	           
	            edge [bend right]  node {} (G)
	            edge [bend right]  node {} (F)
	            
	            (R) 
	            edge [bend left]  node {} (P)
	           
	            edge [bend right]  node {} (G)
	            edge [bend right]  node {} (F);
	          
	            
	  \path[edge]
	         (A) 
	            edge  node {} (O)
	        
	        (E) edge   node {} (A)
	            edge  node {} (Q)
	      
	         (F)
	            edge   node {} (Q)
	        
	            edge   node {} (NJ)
	            
	         (G)edge  node {} (O)
	           
	            
	            edge   node {} (N)
	            
	          (H)edge  node {} (A)
	         
	            
	          (I)
	            edge   node {} (C)
	    
	            edge   node {} (F)
	            edge  node {} (E)
	          
	          (J) 
	           
	            edge   node {} (K)
	            
	         (K)edge  node {} (A)
	            edge   node {} (Q)
	         
	            edge  node {} (NJ)
	          
	          (L)  edge   node {} (Q)
	           
	             edge   node {} (Q)
	            edge   node {} (F)
	
	         (M) edge   node {} (B)
	            edge   node {} (C)
	      
	 
	          (X)
	          edge   node {} (C)
	            edge   node {} (D)
	         
	          
	          (Y)  edge   node {} (Q)
	            edge   node {} (F);
	         
	            
	            
	        
	\end{tikzpicture}
	\end{minipage}
	\hspace{0.5cm}
	& \begin{minipage}{0.05\textwidth}
	
	\usetikzlibrary{arrows}
	\begin{center}
	%\text{Predicting missing edges}
	
	\begin{tikzpicture}
	    \draw[
	        -triangle 60,
	        line width=1mm,
	        postaction={draw, line width=0.2cm, shorten >=0.3cm, -}
	    ] (0,0) -- (1,0);
	\end{tikzpicture}
	\end{center}
	
	\end{minipage}
	
	&\begin{minipage}{0.15\textwidth}
	\begin{tikzpicture}[->,auto,node distance=2.0cm, thick]
	                    
	  \tikzstyle{every state}=[fill=orange,draw=none,text=white, scale=0.25]
	  \tikzstyle{blue edge} = [draw,line width=0.25pt,blue]
	  \tikzstyle{edge} = [draw,line width=0.25pt,green]
	
	  \node[state] (A)                    {};
	  \node[state]         (B) [above right of=A] {};
	  \node[state]         (D) [below right of=A] {};
	  \node[state]         (C) [below right of=B] {};
	  \node[state]         (E) [below of=D]       {};
	  \node[state]         (F) [right of=D]       {};
	  \node[state]         (G) [below of=B]       {};
	  \node[state]         (H) [below right of=D] {};
	  \node[state]         (I) [below right of=H] {};
	  \node[state]         (J) [above right of=I] {};
	  \node[state]         (K) [above right of=C] {};
	  \node[state]         (L) [right of=C] {};
	  \node[state]         (M) [below right of=J] {};
	  \node[state]         (N) [ right of=M] {};
	  \node[state]         (NJ)[above right of=N] {};
	  \node[state]         (O) [above  of=NJ] {};
	  \node[state]         (P) [above left of=O] {};
	  \node[state]         (Q) [below left of=P] {};
	  \node[state]         (R) [above of=P] {};
	  \node[state]         (X) [below of=Q] {};
	  \node[state]         (Y) [left of=R] {};
	  
	  %\draw (A)--(Q);
	
	  \path (A) [blue edge]  [bend left]    node {} (B)
	            edge [bend left]  node {} (C)
	            edge [bend left]  node {} (D)
	           
	            edge [bend left]  node {} (I)
	            edge [bend left]  node {} (Q)
	            edge [bend right]  node {} (L)
	        (B) edge [bend left]  node {} (C)
	            
	            edge [bend left]  node {} (I)
	            edge [bend left]  node {} (Q)
	            edge [bend right]  node {} (L)
	            
	            edge [bend left]  node {} (C)
	            edge [bend left]  node {} (D)
	            edge [bend right]  node {} (G)
	            edge [bend right]  node {} (F)
	        (C) edge [bend left]  node {} (D)
	            
	            edge [bend left]  node {} (P)
	            edge [bend left]  node {} (I)
	            edge [bend left]  node {} (Q)
	            edge [bend left]  node {} (O)
	            edge [bend left]  node {} (K)
	            edge [bend right]  node {} (NJ) 
	        (D) edge [bend left]  node {} (A)
	            edge [bend right]  node {} (P)
	            edge [bend right]  node {} (I)
	            edge [bend right]  node {} (Q)
	            edge [bend left]  node {} (O)
	            edge [bend left]  node {} (M)
	            edge [bend right]  node {} (NJ)
	            
	         (E) edge [bend right]  node {} (P)
	            edge [bend right]  node {} (I)
	            edge [bend right]  node {} (Q)
	            edge [bend left]  node {} (O)
	            edge [bend left]  node {} (M)
	            edge [bend right]  node {} (NJ)
	            edge [bend left]  node {} (C)
	            edge [bend left]  node {} (D)
	            edge [bend right]  node {} (G)
	            edge [bend right]  node {} (F)
	          (F) edge [bend right]  node {} (P)
	            edge [bend right]  node {} (I)
	            edge [bend right]  node {} (Q)
	            edge [bend left]  node {} (O)
	            edge [bend left]  node {} (M)
	            edge [bend right]  node {} (NJ)
	          (G)
	            edge [bend left]  node {} (A)
	            edge [bend left]  node {} (B)
	            edge [bend left]  node {} (C)
	            edge [bend left]  node {} (D)
	            edge [bend left]  node {} (F)
	            edge [bend left]  node {} (NJ)
	            
	            (H)
	             edge [bend left]  node {} (C)
	            edge [bend left]  node {} (D)
	            edge [bend left]  node {} (Y)
	            
	          (I) edge [bend left]  node {} (A)
	            edge [bend left]  node {} (B)
	            edge [bend left]  node {} (C)
	            edge [bend left]  node {} (D)
	            edge [bend left]  node {} (F)
	            edge [bend left]  node {} (NJ)
	            edge [bend left]  node {} (C)
	            edge [bend left]  node {} (D)
	            edge [bend right]  node {} (G)
	            edge [bend right]  node {} (F)
	            
	            (J)  edge [bend left]  node {} (C)
	            edge [bend left]  node {} (D)
	            
	            (K) edge [bend left]  node {} (A)
	            edge [bend left]  node {} (P)
	            edge [bend left]  node {} (C)
	            edge [bend left]  node {} (G)
	            edge [bend left]  node {} (H)
	            edge [bend left]  node {} (NJ)
	            edge [bend left]  node {} (C)
	            edge [bend left]  node {} (D)
	            edge [bend right]  node {} (G)
	            edge [bend right]  node {} (F)
	            edge [bend left]  node {} (Y)
	            
	            (L)  edge [bend left]  node {} (C)
	            edge [bend left]  node {} (D)
	            edge [bend left]  node {} (Y)
	            
	            (NJ)  edge [bend left]  node {} (G)
	            edge [bend left]  node {} (H)
	            (O)  edge [bend left]  node {} (C)
	            edge [bend left]  node {} (D)
	            
	            (N)  edge [bend left]  node {} (P)
	            edge [bend left]  node {} (Y)
	            
	            (M) edge [bend left]  node {} (G)
	            edge [bend left]  node {} (H)
	            edge [bend left]  node {} (NJ)
	            edge [bend left]  node {} (C)
	            edge [bend left]  node {} (D)
	            edge [bend right]  node {} (G)
	            edge [bend right]  node {} (F)
	            edge [bend left]  node {} (Y)
	            
	            (R) edge [bend left]  node {} (A)
	            edge [bend left]  node {} (P)
	            edge [bend left]  node {} (C)
	            edge [bend left]  node {} (G)
	            edge [bend left]  node {} (H)
	            edge [bend left]  node {} (NJ)
	            edge [bend left]  node {} (C)
	            edge [bend left]  node {} (D)
	            edge [bend right]  node {} (G)
	            edge [bend right]  node {} (F);
	          
	            
	  \path[edge]
	         (A) edge  node {} (Q)
	            edge  node {} (O)
	            edge   node {} (M)
	            edge   node {} (NJ)
	            edge  node {} (R)
	            edge  node {} (X)
	            edge   node {} (Y)
	            edge   node {} (K)
	        (E) edge   node {} (A)
	            edge  node {} (Q)
	            edge  node {} (O)
	            edge   node {} (M)
	            edge   node {} (NJ)
	         (F) edge   node {} (A)
	            edge   node {} (Q)
	            edge   node {} (O)
	            edge   node {} (M)
	            edge   node {} (NJ)
	            
	         (G)edge  node {} (O)
	            edge   node {} (P)
	            edge   node {} (Q)
	            edge   node {} (M)
	            edge   node {} (N)
	            
	          (H)edge  node {} (A)
	            edge   node {} (Q)
	            edge   node {} (O)
	            edge   node {} (M)
	            edge  node {} (NJ)
	            
	          (I)edge   node {} (A)
	            edge   node {} (B)
	            edge   node {} (C)
	            edge   node {} (D)
	            edge   node {} (G)
	            edge   node {} (F)
	            edge  node {} (E)
	          
	          (J) edge  node {} (Q)
	            edge  node {} (O)
	            edge   node {} (M)
	            edge   node {} (NJ)
	            edge  node {} (R)
	            edge  node {} (X)
	            edge   node {} (Y)
	            edge   node {} (K)
	            
	         (K)edge  node {} (A)
	            edge   node {} (Q)
	            edge   node {} (O)
	            edge   node {} (M)
	            edge  node {} (NJ)
	          
	          (L)  edge   node {} (Q)
	            edge   node {} (O)
	            edge   node {} (M)
	            edge  node {} (NJ)
	             edge   node {} (Q)
	            edge   node {} (F)
	            edge   node {} (G)
	            edge  node {} (L)
	            
	         (M) edge   node {} (B)
	            edge   node {} (C)
	            edge   node {} (D)
	            edge   node {} (G)
	            edge   node {} (F)
	            edge  node {} (E)
	            
	          (X)
	          edge   node {} (C)
	            edge   node {} (D)
	            edge   node {} (G)
	            edge   node {} (F)
	            edge  node {} (E)
	          
	          (Y)  edge   node {} (Q)
	            edge   node {} (F)
	            edge   node {} (G)
	            edge  node {} (L);
	           
	            
	            
	        
	\end{tikzpicture}
	
	\end{minipage}
	\end{tabular} 
	


==> moreXAIP.tex <==
\section{Making Planning More Explainable}

\dan{Perhaps this section could be merged with section 6 ?}



==> planning.tex <==
\section{Predictions in the Planning Problem}\label{sec:pla}

In this section we describe in detail the problem of state prediction.

\begin{definition}[Planning Problem]
A planning instance $\Pi$ is a pair $\langle D, P \rangle$, where domain $D=\langle S, A, arity \rangle$ is a tuple consisting of a finite set of predicate symbols $Pred$, a finite set of (durative) actions $A$, and a function $arity$ mapping all symbols in $Pred$ to their respective arities. The triple describing problem $P = \langle O, s', G \rangle$ consists of a finite set of domain objects $O$, the partial state $s'$, and the goal specification $G$.
\end{definition}

The atoms of the planning instance are the (finitely many) expressions formed by grounding; applying the predicate symbols $Pred$ to the objects in $O$ (respecting arities). The resultant expressions are the set of propositions $Prop$.

A state $s$ is described by a set of literals formed from the propositions in $Prop$, $\{l_p, \neg l_p, \forall p \in Prop\}$. If every proposition from $Prop$ is represented by a literal in the state, then we say that $s$ is a \textit{complete state}.

A \textit{partial state} is a set of literals $s'\subset s$, where $s$ is a complete state. A partial state $s'$ can be \textit{extended} into a more complete state $s''$ by adding literals.

\begin{definition}[Extending a Partial State]
Let $s'$ be a partial state of Planning problem $\Pi$. 
Extending the state $s'$ is a function $Extend(\Pi,s') : s' \rightarrow s''$ where $s'\subseteq s''$ and $s''\subseteq s$.
\end{definition}

We describe a processing step implementing $Extend$. In order to be able to apply a machine learning technique to extend an incomplete state, we first translate it to a multigraph. Thus, the function $Extend(\Pi,s')$ is implemented as follows: (1) the partial state $s'$ is converted into a multigraph; (2) edges in the multigraph are learned using \MMMVR; (3) the new edges are added as literals to the partially-known state. 

\subsection{Constructing the Multigraph}

We represent a partially-known state $s'$ as a partially-known multigraph $M'$.

\begin{definition}[Partially-known Multigraph]
A partially-known multigraph $M'$ is a pair $\langle V, E' \rangle$, where $V$ is a set of vertices, and $E'$ a set of values of directed edges.
\end{definition}

The values assigned to all possible edges are $\lbrace 0,1,?\rbrace$ corresponding to 
$\lbrace \textit{not-existing},\textit{existing}, \textit{unknown} \rbrace$.
We use $E'$ to denote a set of edge values in a partially-known multigraph, while $E$ denotes the set of edges values in a completed multigraph $M$. 
The partial state $\textit{s'}$ is described as a partially-known multigraph with an edge for each proposition $p\in P$ that is either unknown or known to be true. That is:

\begin{equation}
\label{eq:multigraphdef}
\begin{array}{lcl}
V &\equiv& O \\
E' &=& \{ e_{pred}(b,u) | (b,u)\in V \times V \}
\end{array}
\end{equation}


The existence of a \textit{directed edge} $e_{pred}(b,u)$ between two vertices $b$ and $u$ for a predicate $pred$ is described by the function $L_{pred} : V \times V \rightarrow \{0,1,?\}$. Edges are directed in the order the object symbols appear in the proposition.

For example, let $b$ and $u$ be two vertices in set $V$. For proposition $p$ involving objects $b$ and $u$, $L_{pred}(b,u)=0$ if $\neg l_p\in s'$, $L_{pred}(b,u)=1$ if $l_p\in s'$, and $L_{pred}(b,u)=?$ otherwise.

For an origin object $b$ and a destination object $u$, we define the \textit{edge-vector} as the vector:
$$
\mathbf{e}_{bu} = \left[ L_{pred}(b,u), \forall pred\right]
$$
This vector describes the existence of all edges directed from $b$ to $u$. This is illustrated in an example below.

%\commentS{Remove this completely, move to conclusion perhaps} 
%If required by the domain, predicates without any object parameters can be represented by a virtual vertex, with a single looping edge representing the proposition.

\subsection{Example}

Consider the problem where a robot is able to move between waypoints, pick up, push, and manipulate objects, and put them in boxes. The predicates \texttt{can-pickup}, \texttt{can-push}, \texttt{can-stack-on}, and \texttt{can-fit-inside} describe whether it is possible to perform certain actions upon objects in the environment.

In this problem we restrict our attention to four objects: \texttt{robot}, \texttt{cup01}, \texttt{box01}, and \texttt{block01}. 
In PDDL 2.1~\cite{fox03} literals that are absent from the state are assumed to be false.  However, we assume those literals to be unknown.

 A graph $M$ is generated, the vertices of which are $O:=\{robot, cup01, box01, block01\}$ (Figure \ref{fig:problem}). 
An edge-vector example in this graph is given with:

$$
\begin{array}{l}
\mbf{e}_{robot,block01} 
=  \\
\qquad  \left[ 
\begin{array}{l}
L_{can-fit-inside}(robot,block01) \\
L_{can-stack-on}(robot,block01) \\
L_{can-push}(robot,block01) \\
L_{can-pickup}(robot,block01) \\
\end{array} 
\right] 
=
\left[ 
\begin{array}{l}
0 \\
0 \\
1 \\
? \\
\end{array} \right]
\end{array}
$$

This example edge-vector describes the edge between the nodes \textit{robot} and \textit{block01}. In the example state it is known that the propositions \texttt{(can-fit-inside robot block01)} and \texttt{(can-stack-on robot block01)} are false. It is also known that the proposition \texttt{(can-push robot block01)} is true. Finally, \texttt{(can-pickup robot block01)} is unknown.

\begin{figure}
\vspace{2em}
\begin{center}
\includegraphics[width=0.5\textwidth]{img/translatetograph.pdf}
\end{center}
\caption{A fragment of an example problem from the \texttt{tidy-room} domain translated to the multigraph. Known edges are denoted by solid lines and unknown ones by dashed lines.}
\label{fig:problem}
\end{figure}


